Topological kicks enhance colloidal diffusivity in topological turbulence

Colloidal inclusions in nematic fluids induce topological defects that govern their dynamics. These defects create well-understood rheological behavior in passive nematics, but the interplay between colloid-associated defects and spontaneously generated activity-induced defects introduces new dynamical regimes in active nematic turbulence. Using mesoscale simulations, we study the motion of colloids with strong anchoring in an active nematic and find effective colloid diffusivity exhibits a striking non-monotonic dependence on activity. At low activities, topological kicks from the motile activity-induced bulk defects drive frequent rearrangements of the colloid-associated defects, enhancing colloidal transport. At high activity, defect interactions become isotropic, decorrelating colloidal motion and reducing the effective diffusivity. Our results reveal how the competition between colloid-associated and activity-induced defects fundamentally shapes transport in active nematics.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
